High-Speed Generation of Periodic Traffic Patterns on P4TG for DDoS and Burst-Load Evaluation

Traffic generators are essential tools for evaluating the robustness and performance of networked systems. P4TG is an open-source, hardware-accelerated traffic generator implemented in P4 for the Intel Tofino ASIC. It has been adopted by researchers and industry due to its flexibility and multi-terabit generation capability, and its low cost compared to other traffic generators. However, like most existing generators, it primarily produces constant bit rate traffic, which does not reflect the highly time-varying behavior observed in real networks, such as flashcrowds and microbursts. Such patterns are difficult to emulate at scale with current tools. We present a data plane mechanism for P4TG that shapes periodic, time-varying traffic patterns, including patterns representative of DDoS attacks and burst-load scenarios. Pattern shaping in P4TG can be applied to its generated traffic at an aggregate throughput of up to 4 Tbit/s. We evaluate pattern accuracy and analyze scalability across different sampling resolutions and periods. Further, we demonstrate practical use cases, including zero-loss throughput determination and buffer capacity measurement. Finally, we present microburst-based attack scenarios that overload UDP receivers, switch buffers, and degrade TCP throughput on shared links while remaining undetectable to conventional rate monitoring.

==> chapters/06-discussion.tex <==
\section{Discussion}
\label{sec:discussion}
In this section, we discuss limitations of the pattern shaping introduced for P4TG in this work and outline opportunities for future extensions.

First, while P4TG supports various Layer~2 and Layer~3 encapsulations, it currently generates only UDP traffic at Layer~4.
While this is sufficient for backbone-level testing, simulating CDN-related \ac{DDoS} attacks often requires TCP traffic.
Implementing full TCP behavior is difficult in P4 because of the protocol’s statefulness.
A possible extension is to replace the UDP encapsulation with TCP headers, similar to PIPO-TG~\cite{CoVo24}, although this does not reproduce real TCP state.
Second, P4TG does currently not support application-layer payloads, because its measurement metadata, i.e., timestamps and sequence numbers, is encapsulated in the UDP payload.
Removing this measurement header would allow generating application-layer traffic, but at the cost of the integrated \ac{RTT} and packet-loss measurement functionality.
We plan to explore mechanisms that support both payloads and measurement metadata in future work.
Finally, P4TG’s current implementation averages TX/RX rates over 1-second intervals, consistent with common monitoring tools like SNMP~\cite{rfc3410} and NetFlow~\cite{rfc3176}.
While this limits the direct observability of short-lived microbursts in the exported rate measurements, it does not constrain the generation of sub-second or microsecond-scale traffic patterns.
Instead, this behavior reflects real-world operational monitoring practices and highlights the need for high-resolution measurement systems in production environments.
Improving this granularity or combining P4TG with external measurement systems, such as P4STA~\cite{KuSi20} with its microburst-detection features, may provide finer insights into short-lived traffic behavior.

Beyond these limitations, P4TG is designed to be extensible.
While the system currently implements four shaping functions, additional traffic patterns can be added easily in the control plane as mathematical functions.
Further, pattern shaping enables more efficient execution of existing benchmarking procedures.
For example, zero-loss throughput tests, as defined in RFC 2544~\cite{rfc2544},  require repeated start–stop reconfiguration to iteratively determine the throughput.
With pattern shaping, a single sawtooth pattern can continuously increase the rate to determine zero-loss throughput in a single run, as applied in \sect{eval_throughput}.
